FastMapSVM: Classifying Complex Objects Using the FastMap Algorithm and Support-Vector Machines

Neural Networks and related Deep Learning methods are currently at the leading edge of technologies used for classifying objects. However, they generally demand large amounts of time and data for model training; and their learned models can sometimes be difficult to interpret. In this paper, we advance FastMapSVM -- an interpretable Machine Learning framework for classifying complex objects -- as an advantageous alternative to Neural Networks for general classification tasks. FastMapSVM extends the applicability of Support-Vector Machines (SVMs) to domains with complex objects by combining the complementary strengths of FastMap and SVMs. FastMap is an efficient linear-time algorithm that maps complex objects to points in a Euclidean space while preserving pairwise domain-specific distances between them. We demonstrate the efficiency and effectiveness of FastMapSVM in the context of classifying seismograms. We show that its performance, in terms of precision, recall, and accuracy, is comparable to that of other state-of-the-art methods. However, compared to other methods, FastMapSVM uses significantly smaller amounts of time and data for model training. It also provides a perspicuous visualization of the objects and the classification boundaries between them. We expect FastMapSVM to be viable for classification tasks in many other real-world domains.

==> figures/hyperplane/hyperplane.tex <==
\begin{figure}
	\centering
	\resizebox{\textwidth}{!}{%
		\begin{tikzpicture}[
		x  = {(2cm,0cm)},
		y  = {(-1cm,-1.5cm)},
		z  = {(0cm,2cm)}
		]
		\newcommand{\oax}{1.5}
		\newcommand{\oay}{0.5}
		\newcommand{\oaz}{0.75}
		
		\newcommand{\obz}{2.5}
		
		\newcommand{\oix}{1}
		\newcommand{\oiy}{1.5}
		\newcommand{\oiz}{2}
		
		\newcommand{\ojx}{3.5}
		\newcommand{\ojy}{1.}
		\newcommand{\ojz}{1.5}
		
		\draw[thick]
		(0,0,0) --
		(4,0,0) --
		(4,2,0) --
		(0,2,0) node[anchor=south west, pos=0.95]{\LARGE{$\mathcal{H}$}} --
		cycle;
		
		% Draw the line connecting Oa and Ob
		\draw
		(\oax, \oay, \oaz) node[circle, fill=black, inner sep=0pt, minimum size=3pt,label=right:{$O_a$}]{} --
		(\oax, \oay, \obz) node[circle, fill=black,  inner sep=0pt, minimum size=3pt,label=right:{$O_b$}]{};
		
		% Draw the projection of Oa and Ob on H
		\draw[dashed]
		(\oax, \oay, \oaz) --
		(\oax, \oay, 0) node[circle, fill=black,  inner sep=0pt, minimum size=3pt]{};
		
		\draw
		(\oix, \oiy, \oiz) 
		node[circle, fill=black,  inner sep=0pt, minimum size=3pt,label=left:{$O_i$}]{} 
		-- (\oax, \oay, \oiz)
		node[circle, fill=black,  inner sep=0pt, minimum size=3pt]{}
		-- (\ojx, \ojy, \ojz)
		-- cycle;
		
		\draw
		(\ojx, \ojy, \ojz) 
		node[circle, fill=black,  inner sep=0pt, minimum size=3pt,label=right:{$O_j$}]{} 
		-- (\oax, \oay, \ojz) 
		node[circle, fill=black,  inner sep=0pt, minimum size=3pt]{}
		-- (\oix, \oiy, \ojz)
		node[circle, fill=black,  inner sep=0pt, minimum size=3pt]{}
		-- cycle;
		
		% Project Oi onto H
		\draw[dashed]
		(\oix, \oiy, \oiz) 
		-- (\oix, \oiy, 0)
		node[circle, fill=black,  inner sep=0pt, minimum size=3pt, label=left:{$O_i^\prime$}]{};
		
		% Project Oj onto H
		\draw[dashed]
		(\ojx, \ojy, \ojz) 
		-- (\ojx, \ojy, 0)
		node[circle, fill=black,  inner sep=0pt, minimum size=3pt, label=right:{$O_j^\prime$}]{};
		
		% Connect Oi' and Oj'
		\draw
		(\oix, \oiy, 0) -- (\ojx, \ojy, 0);
		\draw[dashed]
		(\oix, \oiy, 0) -- (\oax, \oay, 0) -- (\ojx, \ojy, 0);
		
		\end{tikzpicture}
	}
	\caption{Hyperplane}
	\label{fig:hyperplane}
\end{figure}
